CLAWSAT: Towards Both Robust and Accurate Code Models

We integrate contrastive learning (CL) with adversarial learning to co-optimize the robustness and accuracy of code models. Different from existing works, we show that code obfuscation, a standard code transformation operation, provides novel means to generate complementary `views' of a code that enable us to achieve both robust and accurate code models. To the best of our knowledge, this is the first systematic study to explore and exploit the robustness and accuracy benefits of (multi-view) code obfuscations in code models. Specifically, we first adopt adversarial codes as robustness-promoting views in CL at the self-supervised pre-training phase. This yields improved robustness and transferability for downstream tasks. Next, at the supervised fine-tuning stage, we show that adversarial training with a proper temporally-staggered schedule of adversarial code generation can further improve robustness and accuracy of the pre-trained code model. Built on the above two modules, we develop CLAWSAT, a novel self-supervised learning (SSL) framework for code by integrating $\underline{\textrm{CL}}$ with $\underline{\textrm{a}}$dversarial vie$\underline{\textrm{w}}$s (CLAW) with $\underline{\textrm{s}}$taggered $\underline{\textrm{a}}$dversarial $\underline{\textrm{t}}$raining (SAT). On evaluating three downstream tasks across Python and Java, we show that CLAWSAT consistently yields the best robustness and accuracy ($\textit{e.g.}$ 11$\%$ in robustness and 6$\%$ in accuracy on the code summarization task in Python). We additionally demonstrate the effectiveness of adversarial learning in CLAW by analyzing the characteristics of the loss landscape and interpretability of the pre-trained models.

==> 8figures_tables.tex <==
%<*tab:generalization-robustness>

\begin{table*}[htb]
    %\centering
    %{
    \setcounter{table}{1}
    \renewcommand{\arraystretch}{1.4}%
    \begin{adjustbox}{max width=2\columnwidth,center}
    \begin{tabular}{cl|cc|cc|cc|cc|cc|cc|cc|cc}
         & ~ & \multicolumn{4}{c|}{\textbf{\summarypy}} & \multicolumn{4}{c|}{\textbf{\summaryjava}} & \multicolumn{4}{c|}{\textbf{\completepy}} & \multicolumn{4}{c}{\textbf{\clonejava}} \\
         \multicolumn{2}{c|}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c}{\textbf\robf}\\
         \hline
         \modelnum{1} & %\notate{\fullysup}{\ff}{\stdtr} 
         Supervised learning & \multicolumn{2}{c|}{${33.33}_{\pm 0.17}$} & \multicolumn{2}{c|}{$26.16_{\pm 0.31}$} &  \multicolumn{2}{c|}{$38.42_{\pm 0.25}$}   & \multicolumn{2}{c|}{$29.89_{\pm 0.27}$} & \multicolumn{2}{c|}{${56.72_{\pm 0.22}}$}  & \multicolumn{2}{c|}{$53.89 _{\pm 0.26}$}& \multicolumn{2}{c|}{$67.20_{\pm 0.11}$} &  \multicolumn{2}{c}{$64.35_{\pm 0.15}$} \\
         \modelnum{2} & \notate{\modelnum{1}}{\ff}{\advtr} \cite{ramakrishnan2020} &\multicolumn{2}{c|}{${33.03}_{\pm 0.21}$}  & \multicolumn{2}{c|}{${32.20}_{\pm 0.26}$} & \multicolumn{2}{c|}{${37.81}_{\pm 0.23}$}  &\multicolumn{2}{c|}{${34.86}_{\pm 0.29}$} & \multicolumn{2}{c|}{${55.40}_{\pm 0.26}$} &\multicolumn{2}{c|}{${55.34}_{\pm 0.35}$} &\multicolumn{2}{c|}{${66.12}_{\pm 0.13}$} & \multicolumn{2}{c}{${65.84}_{\pm 0.17}$} \\
         \modelnum{3} & {\contracode} \cite{jain-etal-2021-contrastive} &\multicolumn{2}{c|}{${36.28}_{\pm 0.18}$}  & \multicolumn{2}{c|}{${28.97}_{\pm 0.27}$} & \multicolumn{2}{c|}{${41.37}_{\pm 0.14}$}  &\multicolumn{2}{c|}{${33.01}_{\pm 0.25}$} & \multicolumn{2}{c|}{${57.70}_{\pm 0.23}$} & \multicolumn{2}{c|}{${54.83}_{\pm 0.31}$} & \multicolumn{2}{c|}{${69.25}_{\pm 0.09}$} &\multicolumn{2}{c}{${68.86}_{\pm 0.13}$} \\\hdashline
        % \modelnum{4} & {\contracode-AT} & 32.80 & ~ & 32.39 & ~ &  38.67 & ~ &  35.91 & ~ & \multicolumn{1}{c}{57.21} & ~ & \multicolumn{1}{c}{56.80} & ~ & \multicolumn{1}{c}{69.20} & ~ & \multicolumn{1}{c}{68.88} & ~\\\hdashline
        % \modelnum{4} & {\notate{\contracode}{\ff}{\advtr}} & \multicolumn{2}{c|}{${35.88}_{\pm 0.20}$} & \multicolumn{2}{c|}{${31.29}_{\pm 0.21}$} &  \multicolumn{2}{c|}{${41.27}_{\pm 0.16}$}  &  \multicolumn{2}{c|}{${38.14}_{\pm 0.24}$} & \multicolumn{2}{c|}{${58.04}_{\pm 0.17}$} & \multicolumn{2}{c|}{${57.01}_{\pm 0.30}$} & \multicolumn{2}{c|}{${69.47}_{\pm 0.10}$} & \multicolumn{2}{c}{${69.08}_{\pm 0.20}$} \\
        %  \modelnum{5} & {\contracode-SAT} & \multicolumn{2}{c|}{${41.01}_{\pm 0.20}$} & \multicolumn{2}{c|}{${39.80}_{\pm 0.21}$} &  \multicolumn{2}{c|}{${41.27}_{\pm 0.16}$}  &  \multicolumn{2}{c|}{${38.14}_{\pm 0.24}$} & \multicolumn{2}{c|}{${58.04}_{\pm 0.17}$} & \multicolumn{2}{c|}{${57.01}_{\pm 0.30}$} & \multicolumn{2}{c|}{${69.47}_{\pm 0.10}$} & \multicolumn{2}{c}{${69.08}_{\pm 0.20}$} \\
        % \modelnum{4} & \notate{\contracode}{\ff}{\advtr} & 32.85 & ~ & 32.56 & ~  & 38.67 & ~ & 35.91 & ~ \\\hdashline
        \modelnum{4} & \notate{\claw}{\ff}{\stdtr} & \multicolumn{2}{c|}{${36.57}_{\pm 0.20}$}  & \multicolumn{2}{c|}{${29.97}_{\pm 0.22}$}  &\multicolumn{2}{c|}{${41.23}_{\pm 0.17}$} & \multicolumn{2}{c|}{${33.53}_{\pm 0.22}$}& \multicolumn{2}{c|}{${57.65}_{\pm 0.25}$} & \multicolumn{2}{c|}{${54.75}_{\pm 0.31}$}  &\multicolumn{2}{c|}{${69.63}_{\pm 0.09}$} &\multicolumn{2}{c}{${68.95}_{\pm 0.15}$} \\
         %(-18.87) (-12.86)
       \modelnum{5} & \notate{\claw}{\ff}{\advtr} & \multicolumn{2}{c|}{${32.97}_{\pm 0.15}$} & \multicolumn{2}{c|}{${32.65}_{\pm 0.17}$} & \multicolumn{2}{c|}{${38.86}_{\pm 0.23}$} & \multicolumn{2}{c|}{${36.10}_{\pm 0.31}$}  & \multicolumn{2}{c|}{${57.44}_{\pm 0.26}$} & \multicolumn{2}{c|}{${57.12}_{\pm 0.29}$} &\multicolumn{2}{c|}{${69.40}_{\pm 0.16}$} &\multicolumn{2}{c}{${69.00}_{\pm 0.14}$}  \\
         %\modelnum{5} & \notate{\ourmodel}{\ff}{\stdtr} & 36.57 & ～ & 29.97 & ~ & 41.23 & ~ & 32.53 & ~ \\
         %\modelnum{6} & \notate{\ourmodel}{\ff}{\advtr} & 32.97 & ~  & 32.65 & ～ & 38.86 & ~ & 36.10 & ～ \\
         %\notate{\ourmodel}{\ff}{\advtrepoch}
         \modelnum{6} & \textbf{{\ourmodel} (ours)} & \multicolumn{2}{c|}{${\mathbf{42.12}}_{\pm 0.19}$} &\multicolumn{2}{c|}{${\mathbf{40.70}}_{\pm 0.23}$} & \multicolumn{2}{c|}{${\mathbf{41.77}}_{\pm 0.27}$} & \multicolumn{2}{c|}{${\mathbf{38.80}}_{\pm 0.33}$} & \multicolumn{2}{c|}{${\mathbf{58.80}}_{\pm 0.24}$}  & \multicolumn{2}{c|}{${\mathbf{57.21}}_{\pm 0.28}$} & \multicolumn{2}{c|}{${\mathbf{69.73}}_{\pm 0.10}$} &\multicolumn{2}{c}{${\mathbf{69.25}}_{\pm 0.13}$} \\
         %$M_{10}$ & \notate{\contracode}{\ff}{\advtrepoch} & 42.06 & ~ & \shash{40.62} & ~ & xx & ~ & xx & ~ \\
    \end{tabular}    
    \end{adjustbox}
    %}
    \caption{{\textbf{Overall performance of \ourmodel}: We evaluate our models in two settings: standard training (\stdtr) and adversarial training (\advtr) by \cite{madry2018towards}. For each of the four tasks: code summarization: \summarypy, \summaryjava, code completion: \completepy, and code clone detection: \clonejava, we report the model's generalization F1-score (\genf) and the robustness F1 (\robf)--the generalization F1 when the model is adversarially attacked. \modelnum{2} corresponds to an adversarially trained (\advtr) version of the supervised model \modelnum{1}, first introduced in \cite{ramakrishnan2020}. \modelnum{4} and \modelnum{5} are two variants of {\ourmodel} (\modelnum{6}): one integrates {\claw} with standard training (\stdtr), and the other integrates {\claw} with the adversarial training (\advtr) \cite{madry2018towards}. The result $ a_{\pm b} $ represents mean $a$ and standard deviation $b$, calculated over $5$ random trials.
    %\SL{[please make analysis and table in the same page.]}
    %\faTrophy~refers to the best performing model for each dataset and metric we report.
    }}
    %~and \faStar
    \label{tab:generalization-robustness}
\end{table*}

%</tab:generalization-robustness>

%<*tab:generalization-robustness2>

\begin{table*}[t!]
    %\centering
    %{
    % \setcounter{table}{2}
    \renewcommand{\arraystretch}{1.4}%
    \begin{adjustbox}{max width=2\columnwidth,center}
    \begin{tabular}{cl|cc|cc|cc|cc|cc|cc|cc|cc}
         & ~ & \multicolumn{4}{c|}{\textbf{\summarypy}} & \multicolumn{4}{c|}{\textbf{\summaryjava}} & \multicolumn{4}{c|}{\textbf{\completepy}} & \multicolumn{4}{c}{\textbf{\clonejava}} \\
         \multicolumn{2}{c|}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c}{\textbf\robf}\\
         \hline
         ~ & {\contracode} \cite{jain-etal-2021-contrastive} &\multicolumn{2}{c|}{${36.28}_{\pm 0.18}$}  & \multicolumn{2}{c|}{${28.97}_{\pm 0.27}$} & \multicolumn{2}{c|}{${41.37}_{\pm 0.14}$}  &\multicolumn{2}{c|}{${33.01}_{\pm 0.25}$} & \multicolumn{2}{c|}{${57.70}_{\pm 0.23}$} & \multicolumn{2}{c|}{${54.83}_{\pm 0.31}$} & \multicolumn{2}{c|}{${69.25}_{\pm 0.09}$} &\multicolumn{2}{c}{${68.86}_{\pm 0.13}$} \\\hdashline
        % \modelnum{2} & {\contracode-AT} & 32.80 & ~ & 32.39 & ~ &  38.67 & ~ &  35.91 & ~ & \multicolumn{1}{c}{57.21} & ~ & \multicolumn{1}{c}{56.80} & ~ & \multicolumn{1}{c}{69.20} & ~ & \multicolumn{1}{c}{68.88} & ~\\\hdashline
        ~ & {\notate{\contracode}{\ff}{\advtr}} & \multicolumn{2}{c|}{${35.88}_{\pm 0.20}$} & \multicolumn{2}{c|}{${31.29}_{\pm 0.24}$} &  \multicolumn{2}{c|}{${38.67}_{\pm 0.27}$}  &  \multicolumn{2}{c|}{${35.91}_{\pm 0.30}$} & \multicolumn{2}{c|}{${57.21}_{\pm 0.19}$} & \multicolumn{2}{c|}{${56.80}_{\pm 0.22}$} & \multicolumn{2}{c|}{${69.20}_{\pm 0.13}$} & \multicolumn{2}{c}{${68.88}_{\pm 0.11}$} \\\hdashline
         ~ & {\contracode-SAT} & \multicolumn{2}{c|}{${41.01}_{\pm 0.20}$} & \multicolumn{2}{c|}{${39.80}_{\pm 0.21}$} &  \multicolumn{2}{c|}{${41.27}_{\pm 0.16}$}  &  \multicolumn{2}{c|}{${38.14}_{\pm 0.24}$} & \multicolumn{2}{c|}{${58.04}_{\pm 0.17}$} & \multicolumn{2}{c|}{${57.01}_{\pm 0.30}$} & \multicolumn{2}{c|}{${69.47}_{\pm 0.10}$} & \multicolumn{2}{c}{${69.08}_{\pm 0.21}$} \\
    \end{tabular}    
    \end{adjustbox}
    %}
    \caption{\small{Effectiveness of {\sat} on {\contracode} 
    }}
    \label{tab:generalization-robustness2}
\end{table*}

%</tab:generalization-robustness2>





% % <*tab:pf-robustness>
% \begin{table}[h]
% % \begin{wrapfigure}[14]{r}{0.5\textwidth}
%     \renewcommand\figurename{Table}
%      \setcounter{figure}{0}
%     {\small
%     \centering
%     {
%     \renewcommand{\arraystretch}{1.35}%
%     %\begin{adjustwidth}{-2cm}{}
%     %\hspace*{-0.8\leftmargin}
%     \resizebox{0.45\textwidth}{!}{
%     \begin{tabular}{p{2.5cm}cc|cc}
%          ~ & \multicolumn{2}{c}{\textbf{\summarypy}} & \multicolumn{2}{c}{\textbf{\summaryjava}}\\
%          \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c}{\textbf\robf}\\
%          \hline
%          %\modelnum{1}: \fullysup & 33.33 & 26.16 & 38.42 & 29.89 \\\hdashline
%         % \notatethree{\contracode}{\pf}{\stdtr}
%         {\small \notate{\contracode}{\pf}{\pf}}
%          & 25.46  &  15.47 & 20.92 & 16.63 \\
%         %\notatethree{\contracode}{\pf}{\advtr} & xx & xx & xx & xx\\
%         %\notate{\ourmodel}{\pf}{\pf}
%         \notate{\claw}{\pf}{\pf}
%         & 25.45  &  19.05 & 22.50 & 17.14 \\\hdashline
%          %\notate{\contracode}{\pf}{\pf}-$5$-\textit{sites} & 25.46  &  15.47 & 20.92 & 16.63 \\
%         %\notatethree{\contracode}{\pf}{\advtr} & xx & xx & xx & xx\\
%         %\notate{\ourmodel}{\pf}{\pf}-$5$-\textit{sites} & 25.45  &  19.05 & 22.50 & 17.14 \\       
%         %\notatethree{\ourmodel}{\pf}{\advtr} & xx & xx & xx & xx \\
        
%           \notate{\contracode}{\ff}{\stdtr} & \multicolumn{1}{c}{36.28}  & \multicolumn{1}{c|}{28.97}  & \multicolumn{1}{c}{41.37}   & \multicolumn{1}{c}{33.01} \\
%      \notate{\claw}{\ff}{\stdtr} & 36.57   & 29.97  & 41.23 & \multicolumn{1}{c}{32.53 }    \\
%         %\\\hdashline
%         %  $M_{5}$ & \notate{\ourmodel}{\pf}{\stdtr} & 25.45 & (-10.83)  &  23.34 & (-5.63) & 22.50 & (-18.87) & 20.15 & (-12.86) \\
%         %  $M_{6}$ & \notate{\ourmodel}{\pf}{\advtr} & xx & ~ & xx & ~ &  xx & ~ &  xx & ~ \\
%        \notate{\contracode}{\ff}{\advtr} & 32.80   & 32.39     & 38.67   & \multicolumn{1}{c}{35.91}    \\
%       \notate{\claw}{\ff}{\advtr} & 32.97   & 32.65 &  38.86   & \multicolumn{1}{c}{36.10}    \\
%     \end{tabular}}
%     }
%     \caption{
%         {\small {Partially fine-tuned (PF) models show that \spc\claw improves robustness. Standard training (\stdtr) yields better generalization than adversarial training (\advtr) while the latter provides better robustness.  \SL{Confusing table as it corresponds to two sub-sections. Needs better separations.}
%         %\spc\genf and {\robf} are the generalization F1-scores and the robust F1-scores, {\ie}, F1 scores of the model when attacked with adversarial codes. These results are on the code summarization task in Python and Java. Details in Section \ref{sec:experiments}.
%         }}
%     }
%     %\caption{\textbf{Pre-training by \spc\claw improves robustness.} Partially fine-tuned models show that \spc\claw improves robustness. \spc\genf and \robf are the generalization F1-scores and the robust F1-scores, {\ie}, F1 scores of the model when attacked with adversarial codes. We evaluate on the \spc\pysmall \cite{sripy} and \spc\javasmall datasets \cite{alon2018general}
%     %\textbf{Generalization and robustness of using different {\ff} schemes}: {\contracode}-{\stdtr} and {\claw}-{\stdtr} refer to the models learned by ST-based FF together with the pre-training method {\contracode} and {\claw}, respectively. {\contracode}-{\advtr} and {\claw}-{\advtr} refer to the models learned by AT-based FF together with {\contracode} and {\claw}, respectively. {\stdtr} results in better generalization than {\advtr} while the latter yields better robustness.} 
%     %However, partial fine-tuning does not improve the \spc\genf of \ourmodel. We study how to co-improve both \spc\genf and \spc\robf of \ourmodel.}
%     %\end{adjustwidth}
%     \label{tab:pf-robustness}
%     }
% \end{table}

% %</tab:pf-robustness>



% <*tab:pf-robustness>
\begin{table}[h]
% \begin{wrapfigure}[14]{r}{0.5\textwidth}
    \renewcommand\figurename{Table}
     \setcounter{figure}{0}
    {\small
    \centering
    {
    \begin{threeparttable}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\hline
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Model\end{tabular}} & \multicolumn{4}{c}{\textbf{Partially fine-tuning }} \\ 
\cline{2-5} & \multicolumn{2}{c|}{\textbf{\summarypy}} & \multicolumn{2}{c}{\textbf{\summaryjava}}\\
\cline{2-5}
~&\multicolumn{1}{c|}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \multicolumn{1}{c|}{\textbf\genf} & \multicolumn{1}{c}{\textbf\robf}\\
\hline
        {\small \notate{\contracode}{\pf}{\pf}}
         & 25.46  &  15.47 & 20.92 & 16.63 \\
        %\notatethree{\contracode}{\pf}{\advtr} & xx & xx & xx & xx\\
        %\notate{\ourmodel}{\pf}{\pf}
        \notate{\claw}{\pf}{\pf}
        & 25.45  &  19.05 & 22.50 & 17.14  \\
        \hline
        ~&\multicolumn{4}{c}{\textbf{Fully fine-tuning and Adversarial fine-tuning }} \\
        \hline
          \notate{\contracode}{\ff}{\stdtr} & \multicolumn{1}{c|}{36.28}  & \multicolumn{1}{c|}{28.97}  & \multicolumn{1}{c|}{41.37}   & \multicolumn{1}{c}{33.01} \\
     \notate{\claw}{\ff}{\stdtr} & 36.57   & 29.97  & 41.23 & \multicolumn{1}{c}{32.53 }    \\
        %\\\hdashline
        %  $M_{5}$ & \notate{\ourmodel}{\pf}{\stdtr} & 25.45 & (-10.83)  &  23.34 & (-5.63) & 22.50 & (-18.87) & 20.15 & (-12.86) \\
        %  $M_{6}$ & \notate{\ourmodel}{\pf}{\advtr} & xx & ~ & xx & ~ &  xx & ~ &  xx & ~ \\
       \notate{\contracode}{\ff}{\advtr} & 32.80   & 32.39     & 38.67   & \multicolumn{1}{c}{35.91}    \\
      \notate{\claw}{\ff}{\advtr} & 32.97   & 32.65 &  38.86   & \multicolumn{1}{c}{36.10}    \\
      \hline
        
        

\end{tabular}

}
% \label{tab:pf-robustness}
\caption{        {{Partially fine-tuned (PF) models show that \spc\claw improves robustness. Standard training (\stdtr) yields better generalization than adversarial training (\advtr) while the latter provides better robustness.  \SL{Confusing table as it corresponds to two sub-sections. Needs better separations.}}}}
\end{threeparttable}
    }
    \caption{
        {\small {Partially fine-tuned (PF) models show that \spc\claw improves robustness. Standard training (\stdtr) yields better generalization than adversarial training (\advtr) while the latter provides better robustness.  \SL{Confusing table as it corresponds to two sub-sections. Needs better separations.}
        %\spc\genf and {\robf} are the generalization F1-scores and the robust F1-scores, {\ie}, F1 scores of the model when attacked with adversarial codes. These results are on the code summarization task in Python and Java. Details in Section \ref{sec:experiments}.
        }}
    }
    %\caption{\textbf{Pre-training by \spc\claw improves robustness.} Partially fine-tuned models show that \spc\claw improves robustness. \spc\genf and \robf are the generalization F1-scores and the robust F1-scores, {\ie}, F1 scores of the model when attacked with adversarial codes. We evaluate on the \spc\pysmall \cite{sripy} and \spc\javasmall datasets \cite{alon2018general}
    %\textbf{Generalization and robustness of using different {\ff} schemes}: {\contracode}-{\stdtr} and {\claw}-{\stdtr} refer to the models learned by ST-based FF together with the pre-training method {\contracode} and {\claw}, respectively. {\contracode}-{\advtr} and {\claw}-{\advtr} refer to the models learned by AT-based FF together with {\contracode} and {\claw}, respectively. {\stdtr} results in better generalization than {\advtr} while the latter yields better robustness.} 
    %However, partial fine-tuning does not improve the \spc\genf of \ourmodel. We study how to co-improve both \spc\genf and \spc\robf of \ourmodel.}
    %\end{adjustwidth}
    \label{tab:pf-robustness}
    }
\end{table}

%</tab:pf-robustness>




%<*tab:transformer>
%\begin{table}[h]
\begin{table}[h!]
    %{
    \centering
    \renewcommand{\arraystretch}{1.4}%
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cl|cc|cc}
         & ~ & \multicolumn{4}{c}{\textbf{\summarypy}}  \\
         \multicolumn{2}{c|}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c}{\textbf\robf} \\
         \hline
         \modelnum{1} & %\notate{\fullysup}{\ff}{\stdtr} 
         Supervised learning & \multicolumn{2}{c|}{${32.60}_{\pm 0.14}$} & \multicolumn{2}{c}{${30.09}_{\pm 0.21}$}   \\
         \modelnum{2} & \notate{\modelnum{1}}{\ff}{\advtr} \cite{ramakrishnan2020} & \multicolumn{2}{c|}{${31.18}_{\pm 0.13}$} & \multicolumn{2}{c}{${30.66}_{\pm 0.23}$}\\
         \modelnum{3} & {\contracode} \cite{jain-etal-2021-contrastive} & \multicolumn{2}{c|}{${34.93}_{\pm 0.11}$} & \multicolumn{2}{c}{${32.86}_{\pm 0.18}$} \\\hdashline
        %\modelnum{5.5} & {\contracode-AT} & 32.80 & ~ & 32.39 & ~ &  38.67 & ~ &  35.91 & ~ & \multicolumn{1}{c}{57.21} & ~ & \multicolumn{1}{c}{56.80} & ~ & \multicolumn{1}{c}{69.20} & ~ & \multicolumn{1}{c}{68.88} & ~\\
         %\modelnum{5.5} & {\contracode-SAT} & 41.01 & ~ & 39.80 & ~ &  41.27 & ~ &  38.14 & ~ & \multicolumn{1}{c}{58.04} & ~ & \multicolumn{1}{c}{57.01} & ~ & \multicolumn{1}{c}{69.47} & ~ & \multicolumn{1}{c}{69.08} & ~ \\\hdashline
        % \modelnum{4} & \notate{\contracode}{\ff}{\advtr} & 32.85 & ~ & 32.56 & ~  & 38.67 & ~ & 35.91 & ~ \\\hdashline
        \modelnum{4} & \notate{\claw}{\ff}{\stdtr} & \multicolumn{2}{c|}{${35.37}_{\pm 0.14}$}  & \multicolumn{2}{c}{${32.31}_{\pm 0.20}$} \\
         %(-18.87) (-12.86)
       \modelnum{5} & \notate{\claw}{\ff}{\advtr} & \multicolumn{2}{c|}{${34.23}_{\pm 0.19}$} & \multicolumn{2}{c}{${33.34}_{\pm 0.18}$}   \\
         %\modelnum{5} & \notate{\ourmodel}{\ff}{\stdtr} & 36.57 & ～ & 29.97 & ~ & 41.23 & ~ & 32.53 & ~ \\
         %\modelnum{6} & \notate{\ourmodel}{\ff}{\advtr} & 32.97 & ~  & 32.65 & ～ & 38.86 & ~ & 36.10 & ～ \\
         %\notate{\ourmodel}{\ff}{\advtrepoch}
         \modelnum{6} & \textbf{{\ourmodel} (ours)} & \multicolumn{2}{c|}{$\mathbf{36.39}_{\pm 0.12}$}  & \multicolumn{2}{c}{$\mathbf{35.53}_{\pm 0.24}$} \\
         %$M_{10}$ & \notate{\contracode}{\ff}{\advtrepoch} & 42.06 & ~ & \shash{40.62} & ~ & xx & ~ & xx & ~ \\
    \end{tabular}    
    \end{adjustbox}
    %}
    \caption{{{Overall performance of {\ourmodel} on transformer}
    %\faTrophy~refers to the best performing model for each dataset and metric we report.
    }}
    %~and \faStar
    \label{tab:transformer}
\end{table}

%</tab:transformer>

%<*generalization-robustness-FF>
%\begin{table}[htb]
% \begin{wrapfigure}[14]{r}{0.45\textwidth}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \renewcommand{\arraystretch}{1.3}%
    \begin{tabular}{lcc|cc}
        ~ & \multicolumn{2}{c}{\textbf{\pysmall}} & \multicolumn{2}{c}{\textbf{\javasmall}}\\
      \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c}{\textbf\robf}\\
         \hline
        %  \modelnum{1} & \notate{\fullysup}{\ff}{\stdtr} & \multicolumn{1}{c}{33.33} & ~ & \multicolumn{1}{c}{22.61} & ~ & \multicolumn{1}{c}{38.42} & ~ & \multicolumn{1}{c}{24.24} & ~ \\
        %  \modelnum{2} & \notate{\fullysup}{\ff}{\advtr} & \multicolumn{1}{c}{33.03} & ~ & \multicolumn{1}{c}{31.42} & ~ & \multicolumn{1}{c}{37.81} & ~ & \multicolumn{1}{c}{23.21} & ~\\
    \notate{\contracode}{\ff}{\stdtr} & \multicolumn{1}{c}{36.28}  & \multicolumn{1}{c|}{28.97}  & \multicolumn{1}{c}{41.37}   & \multicolumn{1}{c}{33.01} \\
     \notate{\claw}{\ff}{\stdtr} & 36.57   & 29.97  & 41.23 & \multicolumn{1}{c}{32.53 } 
         \\\hdashline
        %  $M_{5}$ & \notate{\ourmodel}{\pf}{\stdtr} & 25.45 & (-10.83)  &  23.34 & (-5.63) & 22.50 & (-18.87) & 20.15 & (-12.86) \\
        %  $M_{6}$ & \notate{\ourmodel}{\pf}{\advtr} & xx & ~ & xx & ~ &  xx & ~ &  xx & ~ \\
       \notate{\contracode}{\ff}{\advtr} & 32.85   & 32.56     & 38.67   & \multicolumn{1}{c}{35.91}    \\
      \notate{\claw}{\ff}{\advtr} & 32.97   & 32.65 &  38.86   & \multicolumn{1}{c}{36.10}    \\
        %  \modelnum{7} &\ourmodel & 42.12 & \faTrophy  & 38.10 & \faTrophy & 41.77 & \faTrophy & 36.45 & \faTrophy \\
         %$M_{10}$ & \notate{\contracode}{\ff}{\advtrepoch} & 42.06 & ~ & \shash{40.62} & ~ & xx & ~ & xx & ~ \\
    \end{tabular}
    }
    \caption{\small{\textbf{Generalization and robustness of using different {\ff} schemes}: {\contracode}-{\stdtr} and {\claw}-{\stdtr} refer to the models learned by ST-based FF together with the pre-training method {\contracode} and {\claw}, respectively. {\contracode}-{\advtr} and {\claw}-{\advtr} refer to the models learned by AT-based FF together with {\contracode} and {\claw}, respectively. {\stdtr} results in better generalization than {\advtr} while the latter yields better robustness. 
    %in gen yields a more (or less) significant robustness () improvement
    %\SL{[focus only on PY150?]}
    }}
    \label{tab:generalization-robustness-FF}
    %and \faStar~
%\end{table}
% \end{wrapfigure}
%</generalization-robustness-FF>

%<*tab:weights-epoch-model>
\begin{table}[h]
    {
    \small
    \centering
    \renewcommand{\arraystretch}{1.3}%
    \begin{tabular}{lc}
        \hline
        \multicolumn{1}{c}{$\boldsymbol \theta_{\mathbf\mathrm{\mathrm{pre}}}^\prime$} & \textbf{$||\boldsymbol \theta_{\mathbf\mathrm{\mathrm{pre}}}^\prime-\boldsymbol \theta_{\mathbf\mathrm{\mathrm{pre}}}||_\mathbf{F}$} \\\hline
         \notate{\claw}{\ff}{\stdtr} & 207.99  \\
         \notate{\claw}{\ff}{\advtr} & 323.41  \\
         \ourmodel & ~232.56\\\hdashline
         \notate{\contracode}{\ff}{\stdtr} & 218.14  \\
         \notate{\contracode}{\ff}{\advtr} & 345.36  \\      
          \notate{\contracode}{\ff}{\sat} & 242.70\\\hline
    \end{tabular}
    \caption{
    {Weight difference after finetuning based on different pretraining methods.}
    }
    \label{tab:weights-epoch-model}
    }
\end{table}
%</tab:weights-epoch-model>

%<*lossclaw>
\begin{figure}[htb]
    \centering
    \resizebox{0.45\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/loss_clawsat.png}
    \includegraphics[width=\linewidth]{img/loss_contracode.png}
    }
  \caption{{Loss landscapes:  \spc\claw (L), and  {\contracode} (R), the $\mathbf X$ and $\mathbf Y$ axes represent the directional coefficients $\alpha$ and $\beta$ in  \eqref{eq:losslandscape}.}}
  \label{fig:lossclaw}
%
\end{figure}
%</lossclaw>

%<*finetuning>
\begin{figure}
%\begin{minipage}{\textwidth}%
    \centering
  \resizebox{0.45\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/summary_py_java.png}
  }
  \caption{{Effect of different update schedules ($\tau$, see Algorithm \ref{alg:sat}) on \spc\genf and \robf}}
  \label{fig:robustness-accuracy-epochs}
\end{figure}
%</finetuning>

%<*finetuning-clone>
\begin{figure}[H]
%\begin{minipage}{\textwidth}%
    \centering
  \resizebox{0.45\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/SAT-sch-clone.png}
  }
  \caption{\small{Effect of different update schedules ($\tau$, see Algorithm \ref{alg:sat}) on \spc\genf and \robf}}
  \label{fig:robustness-accuracy-epochs-clone}
 %\end{minipage}
 \end{figure}
%</finetuning-clone>

%<*ebe>
\begin{figure*}[th]
    \centering
\begin{tabular}[htb]{ccc}
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.0\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/ebe1.png}
  }
\end{minipage}%
&
\begin{minipage}{.25\textwidth}%
  \centering
  \resizebox{1.0\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/ebe2.png}
  }
\end{minipage}%
&
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.0\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/ebe3.png}
  }
\end{minipage}%
\\
\multicolumn{1}{p{4.3cm}}{\small{3.a: Sample program from test set (top) and its perturbed variant (bottom)}} & \multicolumn{1}{p{4.3cm}}{\small{3.b: Examples closest to the sample program. Top: \claw, Bottom: \contracode}} & \multicolumn{1}{p{4cm}}{\small{3.c: Examples closest to the perturbed variant. Top: \claw, Bottom: \contracode}}
 \end{tabular}
 \end{figure*}
%</ebe>

%<*ebe2>
\begin{figure*}[th]
    \centering
\begin{tabular}[h]{ccc}
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.2\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/eb4.png}
  }
\end{minipage}%
&
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.0\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/eb5.png}
  }
\end{minipage}%
&
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.1\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/eb6.png}
  }
\end{minipage}%
\\
\multicolumn{1}{p{4.3cm}}{\small{B1.a: Sample program from test set (top) and its perturbed variant (bottom)}} & \multicolumn{1}{p{4.3cm}}{\small{B1.b: Examples closest to the sample program. Top: \claw, Bottom: \contracode}} & \multicolumn{1}{p{4cm}}{\small{B1.c: Examples closest to the perturbed variant. Top: \claw, Bottom: \contracode}}
 \end{tabular}
 \end{figure*}
%</ebe2>
%<*ebe3>
\begin{figure*}[th]
    \centering
\begin{tabular}[h]{ccc}
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.2\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/eb7.png}
  }
\end{minipage}%
&
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{0.9\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/eb8.png}
  }
\end{minipage}%
&
\begin{minipage}{.3\textwidth}%
  \centering
  \resizebox{1.05\textwidth}{!}{
    \includegraphics[width=\linewidth]{img/eb9.png}
  }
\end{minipage}%
\\
\multicolumn{1}{p{4.3cm}}{\small{B1.d: Sample program from test set (top) and its perturbed variant (bottom)}} & \multicolumn{1}{p{4.3cm}}{\small{B1.e: Examples closest to the sample program. Top: \claw, Bottom: \contracode}} & \multicolumn{1}{p{4cm}}{\small{B1.f: Examples closest to the perturbed variant. Top: \claw, Bottom: \contracode}}
 \end{tabular}
 \end{figure*}
%</ebe3>
%<*pretraining1>
\begin{figure}
\centering
\begin{minipage}{.4\textwidth}
  \centering
  \resizebox{0.5\textwidth}{!}{
  \includegraphics[width=\linewidth,valign=t]{img/loss_plot.png}
  }
  \captionof{figure}{A figure}
  \label{fig:test1}
\end{minipage}%
\begin{minipage}{.4\textwidth}
  \centering
  \resizebox{0.5\textwidth}{!}{
  \includegraphics[width=\linewidth,valign=t]{img/loss_plot.png}
  }
  \captionof{figure}{A figure}
  \label{fig:test1}
\end{minipage}%
\begin{minipage}{.4\textwidth}
  \centering
  \figstrut{0.2\linewidth}{0.8\linewidth}
  \renewcommand{\arraystretch}{1.3}%
  \resizebox{0.7\textwidth}{!}{
  \begin{tabular}[t]{ l c }
            \hline
            \multicolumn{1}{c}{$\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime$} & \textbf{$||\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime-\boldsymbol \theta_{\mathbf\mathrm{pre}}||_\mathbf{F}$} \\\hline
             \notate{\claw}{\ff}{\stdtr} & 2538.49  \\
             \notate{\claw}{\ff}{\advtr} & 3518.64  \\
             \ourmodel & ~853.33\\\hline
    \end{tabular}
    }
  \captionof{figure}{Another figure}
  \label{fig:test2}
\end{minipage}
\end{figure}
%</pretraining1>

%<*pretraining2>
\newsavebox{\testbox}%
\newlength{\testheight}%
\savebox{\testbox}{% from https://tex.stackexchange.com/a/66429/121799
        \renewcommand{\arraystretch}{1.3}%
        \begin{tabular}{lc}
            \hline
            \multicolumn{1}{c}{$\boldsymbol\theta_{\mathbf\mathrm{pre}}^\prime$} & \textbf{$||\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime-\boldsymbol \theta_{\mathbf\mathrm{pre}}||_\mathbf{F}$} \\\hline
             \notate{\claw}{\ff}{\stdtr} & 2538.49  \\
             \notate{\claw}{\ff}{\advtr} & 3518.64  \\
             \ourmodel & ~853.33\\\hline
            \end{tabular}
}%
\settoheight{\testheight}{\usebox{\testbox}}
\begin{figure}
\begin{floatrow}
\ffigbox{%
  \includegraphics[height=\testheight]{img/loss_plot.png}%
}{%
  \caption{Q-loud EnrgyCam 2.0}%
}
\ffigbox{%
  \includegraphics[height=2\testheight]{img/loss_plot.png}%
}{%
  \caption{Q-loud EnrgyCam 2.0}%
}
\capbtabbox{%
\usebox{\testbox}
}{%
  \caption{asd}%
}
\end{floatrow}
\end{figure}
%</pretraining2>


%<*tab:weights-epoch-model>
% \begin{wrapfigure}[14]{r}{0.45\textwidth}
%\begin{table}[h]
    {
    \small
    \centering
    \renewcommand{\arraystretch}{1.3}%
    \begin{tabular}{lc}
        \hline
        \multicolumn{1}{c}{$\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime$} & \textbf{$||\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime-\boldsymbol \theta_{\mathbf\mathrm{pre}}||_\mathbf{F}$} \\\hline
         \notate{\claw}{\ff}{\stdtr} & 2538.49  \\
         \notate{\claw}{\ff}{\advtr} & 3518.64  \\
         \ourmodel & ~853.33\\\hline
    \end{tabular}
    \caption{
    \textbf{%{\claw} transfers best to \ourmodel.
    Cross-task transferability assessment through the lens of fine-tuned weights  ($\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime$) versus pre-trained weights ($\boldsymbol \theta_{\mathbf\mathrm{pre}}$). }
    Lower scores suggest better cross-task transferability. The best performance is achieved by {\ourmodel}.
    %of generalization. 
    %from \claw.
    %We compare the weights of three fine-tuned models ($\boldsymbol \theta_{\mathbf\mathrm{pre}}^\prime$) to the weights of \spc\claw ($\boldsymbol \theta_{\mathbf\mathrm{pre}}$).%
    }
    
    \label{tab:weights-epoch-model}
    }
%\end{table}
% \end{wrapfigure}
%</tab:weights-epoch-model>

%<*tab:sensitivity>
% \begin{wrapfigure}[19]{r}{0.65\textwidth}
\begin{table}[ht]
\centering
    \renewcommand{\arraystretch}{1.3}%
    %\hspace*{\leftmargin}
    \small
    \begin{tabular}{lp{9mm}ccc}
     & & \multicolumn{3}{c}{\textbf{Transformations (\genf, \robf)}}\\
    \cline{3-5}
    ~ & ~ & \multicolumn{3}{c}{\textbf{Fine-tuning}}\\
     \multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Pre-training}}}  & ~ & \replace & \insertt & All \\\cline{3-5}
      %\bottomrule
        & {{\replace}} & 41.51, 39.84 &40.49, 34.96 &42.32, 40.75 \\
        & \insertt & 41.71, 40.38 & 41.34, 35.24 & 41.71, 40.38 \\
        & All & 42.66, 40.54 & 41.39, 34.91 & 42.12, 40.70 \\\cline{3-5}
   \end{tabular}
   \\~\\
   %\hspace*{-0.5\leftmargin}
   \begin{tabular}{rccccc} 
         \multirow{1}{*}{\textbf{~}} & \multicolumn{5}{c}{\textbf{Attack strength (\robf)}} \\
         \cline{2-6}
         \multirow{1}{*}{\textbf{~}} & \multicolumn{1}{c}{$\mathbf{1}$} & \multicolumn{1}{c}{$\mathbf{2}$} & \multicolumn{1}{c}{$\mathbf{3}$} & \multicolumn{1}{c}{$\mathbf{4}$} & \multicolumn{1}{c}{$\mathbf{5}$}\\
         \cline{2-6}
         %\modelnum{1}: \fullysup & 33.33 & 26.16 & 38.42 & 29.89 \\\hdashline
        % \notatethree{\contracode}{\pf}{\stdtr}
        {\contracode} &28.97 &28.29 & 27.32 & 26.24& 25.14 \\
         \ourmodel & 40.70  &  40.58 & 39.67 & 38.90 & 38.10\\\cline{2-6}
        %\notatethree{\ourmodel}{\pf}{\advtr} & xx & xx & xx & xx \\
    \end{tabular}
    \caption{\textbf{Performance of \spc\ourmodel at different attack configurations}. We evaluate the sensitivity of our best performing model on (a) different transformation types used during pre-training and fine-tuning (\sat) (b) different attack strengths (number of \sites) during evaluation.
    }
\label{tab:sensitivity}
\end{table}
% \end{wrapfigure}
%</tab:sensitivity>

\begin{comment}
   \begin{tabular}{lp{9mm}ccc}
        & & \multicolumn{3}{c}{\textbf{Attack strength (\genf, \robf)}}\\
        \cline{3-5}
       \multirow{4}{*}{\rotatebox{90}{Pre-training}} &  ~ & \multicolumn{3}{c}{Fine-tuning}\\
      ~ & ~ & $1$ & $3$ & $5$ \\\cline{3-5}
      %\bottomrule
        & \multicolumn{1}{r}{$1$} & 42.08, 40.40 & 42.20, 39.54 & 42.47, 39.87 \\
        & \multicolumn{1}{r}{$3$} & 42.12, 40.70 & 42.26, 39.68 & 42.38, 39.57\\\cline{3-5}
   \end{tabular}
\end{comment}

%<*fig:robustness-accuracy-epochs1>
%\begin{figure}[h]
% \begin{wrapfigure}[12]{r}{0.45\textwidth}
    %\captionsetup[subfigure]{labelformat=empty}
    %\begin{adjustbox}{max width=0.\columnwidth,center}
    \includegraphics[width=\textwidth]{img/gen_rob_acc2.png}
    %\end{adjustbox} 
    \caption{\textbf{Effect of a staggered adversarial code generation schedule during $\mathbf{AT}$}. {X-axis: Epoch-wise frequency of generating adversarial codes. Y-axis: {\genf} or {\robf}.   In the plots, the leftmost point refers to {\modelnum{5}} from  Table \ref{tab:generalization-robustness} which uses adversarial training (\advtr) to generate train-time adversarial codes at every data batch (the most frequent case). Our method {\ourmodel} ({\modelnum{6}}) generates train-time adversarial codes at every epoch.
    }
    % During adversarial training (\advtr), we find that generating adversarial codes at every epoch (model \modelnum{6} from Table \ref{tab:generalization-robustness}) as against at every batch (more frequent; model \modelnum{5}) or at every other epoch (less frequent) provides the best generalization and robustness F1-scores. \spc\advtr by \cite{madry2018towards} has batch-wise updates.
    }
\label{fig:robustness-accuracy-epochs1}
%\end{figure}
% \end{wrapfigure}
%</fig:robustness-accuracy-epochs1>

%<*fig:codeclaw-ssl>
\begin{figure*}[htb]
    \centering
   %\hspace*{-0.0\leftmargin}
    % \begin{adjustbox}{max width=1\textwidth,center}
    % \resizebox{0.5\textwidth}{!}{
    %     \includegraphics[width=\textwidth]{img/transforms.png}
    % }\hfill
    % \resizebox{0.5\textwidth}{!}{
    %     \includegraphics[width=\textwidth]{img/codeclaw_ssl.png}
    % }
    % \hfill
    % %\resizebox{0.6\textwidth}{!}{
    % %    \includegraphics[width=\textwidth]{img/codeclaw_finetuning.png}
    % %}
    % \end{adjustbox}
    \begin{tabular}{cc}
    \hspace*{-0mm}\includegraphics[width=.48\textwidth,height=!]{img/transforms1.png}
    &\hspace*{-0mm}
    \includegraphics[width=.48\textwidth,height=!]{img/codeclaw_ssl1.png} \\
    {(A)} &   {(B)}
\end{tabular}
    \caption{{
    {(A)} Two types of semantics-preserving transformations (obfuscations) can be made to a code to attack code models--{\spc\replace} - where existing code is modified at a \spc\site---location in the code, or {\spc\insertt} - where new lines of code are inserted at a \site. We select \spc\sites at random. The specific tokens used in these transformations (\texttt{test} and \texttt{"Network"} in the the example) can either be a random transformation $t_\text{rand}(\cdot)$--a randomly selected token from a pre-defined vocabulary, or can be an adversarial transformation $t_\text{adv}(\cdot)$, where the token is obtained from solving a first-order optimization designed to fool the model \cite{srikant2021generating,ramakrishnan2020,yefet2020adversarial}.~
    {(B)} During pre-training, we propose \textbf{\claw} containing two optimization problems: (1) to {learn invariant code representations by minimizing the representation distances of a code ($\prog$) from all its views ($t_\text{rand}(\prog)$, $t_\text{adv}(\prog)$) via {\clsmall}}, and (2) to {generate an adversarial code $t_\text{adv}(\prog)$ (`hard' positive example) by  maximizing its representation distance from $\prog$}. In the example, this requires solving for a replacement token at the randomly selected \spc\site marked as \fcolorbox{black}{gblue}{\textbullet}.
    \SL{[Please consider to revise this figure and fit it into one column.]}
    %{(C)} We propose {\textbf{\sat}} - a staggered adversarial training schedule when fine-tuning a model $\mathcal{M}$. The frequency of attacks and updates to the model (line marked \faHashtag~ in the pseudocode describing adversarial training (\advtr)) affects the overall generalization and robustness of the fine-tuned model.
    }}
\label{fig:codeclaw-ssl}
\end{figure*}
%</fig:codeclaw-ssl>


%<*alg:sat>

\begin{algorithm}[htb]
         %\begin{algorithm}
         {\small
            \begin{algorithmic}
        %\resizebox{0.8\textwidth}{!}{
           \STATE {\bfseries Input:} 
           %data batch $\mathcal{B}_i$,
           model $\mathcal{M} = \{ {\boldsymbol \theta_{\mathrm{ft}}, \boldsymbol \theta} \}$, attack frequency $\tau$
          \FOR{each epoch $e$}
                \FOR{each data batch $\mathcal{B}_i$}
                    \STATE  1.~ Train $\mathcal{M}$ by updating $\boldsymbol \theta_{\mathrm{ft}}\circ \boldsymbol \theta$
                \ENDFOR
                \IF{$e$ mod $\tau$ = 0}
                    \FOR{each data batch $\mathcal{B}_i$}
                        \STATE 2.~ Attack $\mathcal{M}$ by finding adversarial codes ${\mathcal B^\prime}_i$
                        %${\mathcal{P^\prime}}_i$
                        % \STATE 3.~ $\mathcal{B^\prime}_i := \mathcal{B}_i \setminus \mathcal{{P^\prime}}_i$ \quad\quad$\rhd$ Update batch
                        \STATE 3.~ Retrain $\mathcal{M}$ on ${\mathcal B^\prime}_i$
                    \ENDFOR
                \ENDIF
           \ENDFOR
           %}
        \end{algorithmic}
        }
        \caption{\small{Staggered Adversarial Training (\sat) %\SL{use wraptable?}
        }}
        \label{alg:sat}
        %\end{algorithm}
\end{algorithm}
%</alg:sat>

%<*alg:sat2>


% \begin{wraptable}%{r}{0.35\textwidth}
%     \begin{tabular}{c}
%     \begin{algorithm}[htb]
%          %\begin{algorithm}
%          {\small
%             \begin{algorithmic}
%         %\resizebox{0.8\textwidth}{!}{
%            \STATE {\bfseries Input:} 
%            %data batch $\mathcal{B}_i$,
%            model $\mathcal{M} = \{ {\boldsymbol \theta_{\mathrm{ft}}, \boldsymbol \theta} \}$, attack frequency $\tau$
%           \FOR{each epoch $e$}
%                 \FOR{each data batch $\mathcal{B}_i$}        
%                     \IF{$e$ mod $\tau$ = 0}
%                     \STATE Generate adversarial codes $\mathcal{B}_i'$
%                     \ENDIF
%                     \STATE Update $\{ {\boldsymbol \theta_{\mathrm{ft}}, \boldsymbol \theta} \}$ with stochastic gradient descent:
%                     \STATE $\quad \quad \mathbf{g}_{\{\boldsymbol \theta_{\mathrm{ft}}, \boldsymbol \theta\}}=\mathbb E_{(\mathbf x, \mathbf y)\in \mathcal{B}_i} \nabla_{\{\boldsymbol \theta_{\mathrm{ft}}, \boldsymbol \theta\}} \ell (\mathbf x, \mathbf y,\boldsymbol \theta_{\mathrm{ft}} \circ \boldsymbol \theta) + \lambda \mathbb E_{(\mathbf x_{adv}, \mathbf y)\in \mathcal{B}_i'} \nabla_{\{ \boldsymbol \theta_{\mathrm{ft}}, \boldsymbol \theta\}} \ell (\mathbf x_{adv}, \mathbf y,\boldsymbol \theta_{\mathrm{ft}} \circ \boldsymbol \theta)$
%                 \ENDFOR
                
%            \ENDFOR
%            %}
%         \end{algorithmic}
%         }
%         \caption{\small{Staggered Adv. Training}}
%         \label{alg:sat2}
%         % \end{algorithm}
% \end{algorithm}
%     \end{tabular}
% \end{wraptable} 
% \begin{wraptable}{cl}

% \end{wraptable}
%</alg:sat2>

%<*tab:generalization-robustness-5-sites>
\begin{table*}[h]
    \centering
    {
    \renewcommand{\arraystretch}{1.3}%
    \begin{tabular}{cl|cc|cc|cc|cc}
         ~ & \multicolumn{1}{c|}{Model} & \multicolumn{4}{c|}{\summarypy} & \multicolumn{4}{c}{\summaryjava} & \multicolumn{4}{c|}{\completepy} & \multicolumn{4}{c|}{\clonejava} \\
         ~ & ~ & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c|}{\textbf\robf} & \multicolumn{2}{c|}{\textbf\genf} & \multicolumn{2}{c}{\textbf\robf}\\
         \hline
         \modelnum{1} & \notate{\fullysup}{\ff}{\stdtr} & \multicolumn{1}{c}{33.33} & ~ & \multicolumn{1}{c}{22.61} & ~ & \multicolumn{1}{c}{38.42} & ~ & \multicolumn{1}{c}{24.24} & ~ \\
         \modelnum{2} & \notate{\fullysup}{\ff}{\advtr} & \multicolumn{1}{c}{33.03} & ~ & \multicolumn{1}{c}{31.42} & ~ & \multicolumn{1}{c}{37.81} & ~ & \multicolumn{1}{c}{23.21} & ~\\
         \modelnum{3} & \notate{\contracode}{\ff}{\stdtr} & \multicolumn{1}{c}{36.28} & ~ & \multicolumn{1}{c}{25.14} & ~ & \multicolumn{1}{c}{41.37} & \faStar & \multicolumn{1}{c}{28.97} & ~\\
         %\modelnum{4} & \notate{\contracode}{\ff}{\advtr} & 35.88 & ~ & 30.60  & \faStar  & 38.67 & ~ & 26.11 & ~ \\\hdashline
        %  $M_{5}$ & \notate{\ourmodel}{\pf}{\stdtr} & 25.45 & (-10.83)  &  23.34 & (-5.63) & 22.50 & (-18.87) & 20.15 & (-12.86) \\
        %  $M_{6}$ & \notate{\ourmodel}{\pf}{\advtr} & xx & ~ & xx & ~ &  xx & ~ &  xx & ~ \\
         \modelnum{5} & \ourmodel-\stdtr & 36.57 & \faStar & 26.52 & ~ & 41.23 & ~ & 28.03 & ~ \\
         \modelnum{6} & \notate{\ourmodel}{\ff}{\advtr} & 36.45 & ~  & 30.03 &  & 38.86 & ~ & 29.00 & \faStar \\
         \modelnum{7} &\ourmodel & 42.12 & \faTrophy  & 38.10 & \faTrophy & 41.77 & \faTrophy & 36.45 & \faTrophy \\
         %$M_{10}$ & \notate{\contracode}{\ff}{\advtrepoch} & 42.06 & ~ & \shash{40.62} & ~ & xx & ~ & xx & ~ \\
    \end{tabular}
    }
    \caption{\textbf{Accuracy and robustness of \ourmodel}: 
    %We evaluate how pre-training and fine-tuning can affect the accuracy \versus robustness trade-off in code models.
    We evaluate our models in two settings: standard training (\stdtr) and adversarial training (\advtr) by \cite{madry2018towards}. For each of the four tasks: code summarization: \summarypy, \summaryjava, code completion: \completepy, and code clone detection: \clonejava, we report the model's generalization F1-score (\genf) and the robustness F1 (\robf)--the generalization F1 when the model is adversarially attacked with $5$ \textit{sites}. 
    %We evaluate the models on the \spc\pysmall and \spc\javasmall datasets. 
    Models \modelnum{1}--\modelnum{4} serve as our baseline (above dotted line); the \spc\contracode model from \cite{jain-etal-2021-contrastive} corresponds to \modelnum{3}. We propose model \modelnum{7} in this work. \faTrophy~refers to the best performing model for each task and metric we report.}
    \label{tab:generalization-robustness-5-sites}
    %and \faStar~
\end{table*}
%</tab:generalization-robustness-5-sites>

%<*tab:Lamb-effect>
\begin{table}[h]
    {
    \centering
    {
    \renewcommand{\arraystretch}{1.2}%
    \begin{tabular}{c|cc|cc|cc|cc|cc}
         \multirow{2}{*}{Model} & \multicolumn{2}{c|}{$\lambda=0.2$} & \multicolumn{2}{c|}{$\lambda=0.4$} & \multicolumn{2}{c|}{$\lambda=0.6$} & \multicolumn{2}{c|}{$\lambda=0.8$}\\
         ~ & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \multicolumn{1}{c}{\textbf\genf} & \multicolumn{1}{c|}{\textbf\robf} & \\
         \hline
         %\modelnum{1}: \fullysup & 33.33 & 26.16 & 38.42 & 29.89 \\\hdashline
        % \notatethree{\contracode}{\pf}{\stdtr}

        \ourmodel & 40.75  &  38.46 & 41.77 & 38.80 & 41.64  &  37.89 & 41.74 & 37.26 \\
        %\notatethree{\ourmodel}{\pf}{\advtr} & xx & xx & xx & xx \\
    \end{tabular}
    }
    \caption{Robustness and generalization varies with different $\lambda$ used in loss function. Our methods with Different $\lambda$ are evaluated on \spc\javasmall.} 
    %However, partial fine-tuning does not improve the \spc\genf of \ourmodel. We study how to co-improve both \spc\genf and \spc\robf of \ourmodel.}
    \label{tab:Lamb-effect}
    }
\end{table}
%</tab:Lamb-effect>

%<*tab:num-sites-effect>
\begin{table}[h]
    {\small
    %\hspace*{-0.5\leftmargin}
    \centering
    {
    \renewcommand{\arraystretch}{1.4}%
    \begin{tabular}{rccccc} 
         \cline{2-6}
         \multirow{1}{*}{\textbf{~}} & \multicolumn{5}{c}{\textbf{Attack strength, \robf}} \\
         \multirow{1}{*}{\textbf{~}} & \multicolumn{1}{c}{$\mathbf{1}$} & \multicolumn{1}{c}{$\mathbf{2}$} & \multicolumn{1}{c}{$\mathbf{3}$} & \multicolumn{1}{c}{$\mathbf{4}$} & \multicolumn{1}{c}{$\mathbf{5}$}\\
         \cline{2-6}
         %\modelnum{1}: \fullysup & 33.33 & 26.16 & 38.42 & 29.89 \\\hdashline
        % \notatethree{\contracode}{\pf}{\stdtr}

          
        {\contracode} &28.97 &28.29 & 27.32 & 26.24& 25.14 \\
         \ourmodel & 40.70  &  40.58 & 39.67 & 38.90 & 38.10\\\cline{2-6}
        %\notatethree{\ourmodel}{\pf}{\advtr} & xx & xx & xx & xx \\
    \end{tabular}
    }
    \caption{\textbf{Varying attack strength at evaluation.} We report the \robf scores of \spc\ourmodel against stronger adversarial attacks during evaluation. The attack strength represents the number of \spc\sites attacked during evaluation.} 
    \label{tab:num-sites-effect}
    }
\end{table}
%</tab:num-sites-effect>
